A Support Vector Model of Pruning Trees Evaluation Based on OTSU Algorithm

The tree pruning process is the key to promoting fruits' growth and improving their productions due to effects on the photosynthesis efficiency of fruits and nutrition transportation in branches. Currently, pruning is still highly dependent on human labor. The workers' experience will strongly affect the robustness of the performance of the tree pruning. Thus, it is a challenge for workers and farmers to evaluate the pruning performance. Intended for a better solution to the problem, this paper presents a novel pruning classification strategy model called "OTSU-SVM" to evaluate the pruning performance based on the shadows of branches and leaves. This model considers not only the available illuminated area of the tree but also the uniformity of the illuminated area of the tree. More importantly, our group implements OTSU algorithm into the model, which highly reinforces robustness of the evaluation of this model. In addition, the data from the pear trees in the Yuhang District, Hangzhou is also used in the experiment. In this experiment, we prove that the OTSU-SVM has good accuracy with 80% and high performance in the evaluation of the pruning for the pear trees. It can provide more successful pruning if applied into the orchard. A successful pruning can broaden the illuminated area of individual fruit, and increase nutrition transportation from the target branch, dramatically elevating the weights and production of the fruits.

==> 6_Conclusion___Discussion.tex <==
\section{Conclusion}
\label{sec:conclusion}
In this paper, the paper designs a support vector machine classification model called OTSU-SVM to evaluate the performance of pruning. It comprehensively measures the features of the fruit trees from two dimensions -- light transmittance dimension and uniformity dimension, and realizes pruning evaluation by integrating these two features and the label of performance.

More importantly, the process of data preprocessing and feature selection plays a significant role before the OTSU-SVM model analysis. We propose three algorithms to preprocess data and measure the feature. The one is to use threshold selection method (OTSU algorithm) to set threshold and determine pixels of the image belong to white or black pixels. The second one is to shrink dimensions and reduce redundancy of the images in order to increase our model efficiency. The last algorithm is to calculate the uniformity of matrix, which is one of features we select. In our method, we define how to measure the black pixels rate and uniformity of shadows. Additionally, we normalize the matrix of features. Normalization is to improve the stability and robustness of the weights of the pruning model. 

The supervised model of machine learning, support vector machine, is used to make a maximum margin hyperplane to classify the good and not good pruning points. Comparing with other pruning decision models, our model has high accuracy and considers more comprehensive factors of the fruit trees. With purpose to prove our model performance, we went to the orchard in Hangzhou, collected the data and took images from pear trees. A dataset is built based on these data and verifies the high accuracy of our model. 

In the future work, we expect these systems can be applied into more areas of agriculture and increase the production of fruits. 


==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************

